TPU as Cryptographic Accelerator

Cryptographic schemes like Fully Homomorphic Encryption (FHE) and Zero-Knowledge Proofs (ZKPs), while offering powerful privacy-preserving capabilities, are often hindered by their computational complexity. Polynomial multiplication, a core operation in these schemes, is a major performance bottleneck. While algorithmic advancements and specialized hardware like GPUs and FPGAs have shown promise in accelerating these computations, the recent surge in AI accelerators (TPUs/NPUs) presents a new opportunity. This paper explores the potential of leveraging TPUs/NPUs to accelerate polynomial multiplication, thereby enhancing the performance of FHE and ZKP schemes. We present techniques to adapt polynomial multiplication to these AI-centric architectures and provide a preliminary evaluation of their effectiveness. We also discuss current limitations and outline future directions for further performance improvements, paving the way for wider adoption of advanced cryptographic tools.

==> sec-ntt-tpu.tex <==

\section{NTT on TPU}\label{sec-ntt-tpu}
Compared with directly multiplication using coefficient representation, NTT using value representation has a lower complexity, which is attractive when the degree of the polynomial is high.

\subsection{NTT and FFT}
Polynomial multiplication using value representation 

The goal of NTT is to convert a polynomial from coefficient representation to value representation.
While this can be easily done by evaluating the polynomial directly on selected values, NTT provides a faster way to do the same job. 
The idea behind NTT (or fast NTT) is exactly the same as FFT (actually fast discrete Fourier transformation, FDFT), which utilizes divide-and-conquer strategy to reduce the computation cost.

\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{fig-fft.png}
    \caption{An example of converting a degree 7 polynomial from coefficient representation to value representation. On the left side, $x(i)$ (column $L_0$) is the coefficient vector and input to the FFT algorithm. On the right side is the output is the value vector $X(i)$ (column $L_3$). Columns $L_1$ and $L_2$ are intermediate results.}
    \label{fig-fft}
\end{figure}

\figurename~\ref{fig-fft} shows the idea of FFT.
Note that on the left size, the coefficients are not provided in the original order, but the ``bit reverse'' order.
The computation is done in three rounds (more generally, $\log_2 n$ rounds where $n-1$ is the polynomial degree), and two sets of intermediate results (vector $L_1$ and $L_2$) are obtained in this process. 
Intuitively, each node of $L_i$ depends on two nodes of $L_{i-1}$.

\subsection{Adopting TPU for NTT Computation}
To utilize TPU for NTT computation, we need to establish a connection between the butterfly transformation given in \figurename~\ref{fig-fft} and matrix multiplication.

